Local Convergence of Gradient Descent-Ascent for Training Generative Adversarial Networks

Generative Adversarial Networks (GANs) are a popular formulation to train generative models for complex high dimensional data. The standard method for training GANs involves a gradient descent-ascent (GDA) procedure on a minimax optimization problem. This procedure is hard to analyze in general due to the nonlinear nature of the dynamics. We study the local dynamics of GDA for training a GAN with a kernel-based discriminator. This convergence analysis is based on a linearization of a non-linear dynamical system that describes the GDA iterations, under an \textit{isolated points model} assumption from [Becker et al. 2022]. Our analysis brings out the effect of the learning rates, regularization, and the bandwidth of the kernel discriminator, on the local convergence rate of GDA. Importantly, we show phase transitions that indicate when the system converges, oscillates, or diverges. We also provide numerical simulations that verify our claims.

==> sections/alt_linearization.tex <==
\section{Alternative Linearization}
Note: for now pretending there is only one generated point.

Given the update function in \cref{eq:Phidef}, the jacobian should be
F := \begin{equation}
    \begin{bmatrix} (1-\lambda \eta_d) & (1-\lambda\eta_d)f'(\x) - \eta_d \mathbb{E}K'(\X,\x) - \eta_d\mathbb{E}K'(\Xt, \x) \\
    \eta_g \pt_j K'(\xt_j,\cdot) & 1+\eta_g\pt_j f'(\xt_j)
    \end{bmatrix}
\end{equation}
Evaluating the Jacobian at $\xt_j = \x_0$ and $f^*(\x)= \frac{1}{\lambda} [\mathbb{E}K(\X,\x) - \mathbb{E}K(\Xt^*,\x)]$ we have
\begin{align}
    F(\z^*) =   \begin{bmatrix} (1-\lambda \eta_d) & 1 \\
    \eta_g \pt_j K'(\x_0,\cdot) & 1
    \end{bmatrix}
\end{align}

==> sections/kernel_generator.tex <==
\section{Kernel Generator}

Consider the setup where the generator is a map $g:\mc Z\to\mc X,$ and $g\in\mc G$ corresponding to the kernel $G$. We focus on $\mc Z=\Real^m$ and $\mc X=\Real^d$ here. We also assume that the latent vectors $z$ that generate samples $\wt x=g(z)$ are drawn from the distribution $\mu=\mc N(0,I_m)$, which is common practice.
Observe that the gradient descent update for the generator model is given by
% \begin{align}
%     g^{t+1} &= g^t + \eta_g\sum_{j=1}^{N_r}\wt p_j \frac{\partial}{\partial g} f^t(g^t(z_j))\\
%     &= g^t + \eta_g \sum_{j=1}^{N_r}\wt p_j\grad f^t(g^t(z_j^t))G(\cdot,z_j^t)
% \end{align}
% 
% In its integral form, this can be stated as
\begin{align}
    g^{t+1} &= g^t + \eta_g\Exp \grad f^t(g^t(Z))G(Z,\cdot)\\
    &= g^t + \eta_g \mc T_g\left\{\grad f^t \circ g^t\right\}
\end{align}
since $\frac{\partial}{\partial g}g^t(z) = G(\cdot, z)$ for all $t.$ Here $\mc T_g: L^2_\mu\to\mc G$ is the integral operator associated with the kernel $G,$ defined as
\begin{align}
    \mc T_g\set{f}(w)=\int G(w,z)f(z)\dif \mu(z)
\end{align}

Assuming $g^t = G(\cdot, \mc Z^{t-1})\betavec^t$.


==> sections/largest_eigenvalue.tex <==
\section{Largest Eigenvalues}
Here let's assume our discriminator learning rate $\eta_d$ is small such that $|\rho|^2\approx1-2\eta_d \text{Re}(s_i)$. The first two eigenvalue magnitudes are
\begin{align}
    |\rho_a|^2 \approx 1-2\eta_d\lambda \nonumber \\
    |\rho_a|^2 \approx 1-2\eta_d\frac{\mu\pt \Delta}{\lambda \sigma^2} \nonumber\\
    |\rho_c|^2\approx 1-\eta_d(\lambda + \frac{\mu\pt \Delta}{\lambda \sigma^2})
\end{align}
When $\rho_c$ has imaginary components its magnitude is approximately:
\begin{equation}
    |\rho_c|^2\approx 1-\eta_d(\lambda + \frac{\mu\pt \Delta}{\lambda \sigma^2})
\end{equation}

==> sections/linear_generator.tex <==
\section{Dynamics for A Linear Generator}

For the linear generator we get the update equation:
\begin{align}
    W_{t+1} = W_{t} - \eta_g\sum_{j=1}^{N_g}\pt_j \grad f(W_t\wt z_j) \wt z_j\tran
\end{align}
Note that this summation is approximating $\mathbb{E}_{\wt z}\left[ \grad f(W_t\wt z) \wt z\tran \right]$, and for a latent vector distribution with zero-mean it is equivalent to the cross-covariance of the latent vector and the gradients. 

If we assume $\wt z_j^t \sim \mc N(0,I)$ for all $t$, then $W_{t+1}=W_t - \eta_g\Exp \grad f_t(W_t Z)Z\tran$. Furthermore by Stien's lemma this simplifies as $\Exp \grad f(W_t Z)Z\tran=\Exp\grad^2 f_t(W_t Z)W_t$
